Machine Reading Comprehension using Case-based Reasoning

We present an accurate and interpretable method for answer extraction in machine reading comprehension that is reminiscent of case-based reasoning (CBR) from classical AI. Our method (CBR-MRC) builds upon the hypothesis that contextualized answers to similar questions share semantic similarities with each other. Given a test question, CBR-MRC first retrieves a set of similar cases from a nonparametric memory and then predicts an answer by selecting the span in the test context that is most similar to the contextualized representations of answers in the retrieved cases. The semi-parametric nature of our approach allows it to attribute a prediction to the specific set of evidence cases, making it a desirable choice for building reliable and debuggable QA systems. We show that CBR-MRC provides high accuracy comparable with large reader models and outperforms baselines by 11.5 and 8.4 EM on NaturalQuestions and NewsQA, respectively. Further, we demonstrate the ability of CBR-MRC in identifying not just the correct answer tokens but also the span with the most relevant supporting evidence. Lastly, we observe that contexts for certain question types show higher lexical diversity than others and find that CBR-MRC is robust to these variations while performance using fully-parametric methods drops.

==> analysis_clustering.tex <==
% \subsection{When is \method\ effective?}
% \subsection{\method\ v/s Latent Relation Frequency and Lexical Diversity}

% \input{zz_fig_latent_rel.tex}

\method\ performs answer extraction 
%operates in a two-step procedure, first filtering the case base using latent relations encoded in the question text followed 
by explicitly comparing span similarities of the target context with the context spans in the filtered casebase. 
Purely parametric methods can also be seen as following a similar mechanism, albeit performing the two steps implicitly. 
These models, therefore, must rely only on the parameter values learned at training in order to handle several relational semantics, which may each be expressed in contexts with varying levels of diversity in language form. In practice, we find that some relations are indeed expressed with more lexical diversity than others (Appendix \ref{app:lex-NQ}). In Figure \ref{fig:lexical-diversity}, we investigate how \method{} performs at inference under varying amounts of lexical diversity observed in passage contexts at \textit{training}. We first cluster questions according to their embeddings and then compute n-gram statistics \citep{li2015diversity, duvsek2020evaluating, tevet2020evaluating} across passage contexts found in each cluster to measure diversity. We use NaturalQuestions as a case study for our analysis and compare performance with BLANC and MADE, two fully-parametric baselines.
% Interestingly, we find that traditional parametric MR methods have lower accuracy as diversity increases, whereas our semi-parametric method maintains high accuracy across relational semantics, particularly under high lexical diversity.
\paragraph{Clustering questions by latent relations.}  We cluster questions in the training set based on the latent relations they encode using hierarchical agglomerative clustering (HAC) \citep{krishna2012efficient} over similarity scores. For a fair evaluation, we compute 6 different flat clusterings of varying cluster tightness, i.e., how similar each question is within a cluster. For each clustering, we compute the per-cluster lexical diversity as the count of the number of unique tokens in the set of passage contexts across questions in the cluster, normalized by the cluster size. We then cluster the test set by assigning each question to the cluster label of its top-1 similar train question for each of the 6 clusterings, resulting in 6 \textit{test} clusterings (see Appendix~\ref{app:lex-clustering} for more details).

\paragraph{Results.} Figure \ref{fig:lexical-diversity} shows the mean F1 scores between \method{} and the baselines on test queries for varying values of lexical diversity observed at training for the same latent relations as the test queries. 
We group clusters by lexical diversity scores into buckets and report the aggregated F1 scores for each bucket.\footnote{(1) We use $k$-means over lexical diversity scores of all clusters to construct $B=8$ buckets. (2) We report the F1 performance on all 6 clusterings in Appendix \ref{app:lex-plots}.}
On average, we find that the performance gap between \method{} and the baselines tends to increase as lexical diversity increases. The min-max F1 difference, which captures the drop in performance as lexical diversity increases, is $4.10$ points for \method{} while BLANC and MADE show significantly larger differences of $15.38$ and $11.80$ points, respectively.
We posit that as diversity in contexts for the same latent relation increases, it is harder for fully parametric models to learn parameters that are suitable for all lexical variations. On the other hand, the semi-parametric nature of \method\ allows it to partially shift this burden to test time and ground itself using only a few retrieved cases that are explicitly compared.

==> related_work.tex <==
\section{Related Work}

\paragraph{Machine Reading Comprehension.} MRC evaluates a machine's ability to reason over natural language by training it to answer questions on a given passage. Several variations of this task exist, such as cloze-style \cite{https://doi.org/10.48550/arxiv.1506.03340,https://doi.org/10.48550/arxiv.1809.00812}, multiple-choice \cite{richardson-etal-2013-mctest,  lai2017large}, extractive \cite{yang-etal-2015-wikiqa, trischler2016newsqa}, and generative question-answering \cite{https://doi.org/10.48550/arxiv.1611.09268, https://doi.org/10.48550/arxiv.1712.07040}.
% \cite{9961260, https://doi.org/10.48550/arxiv.2006.11880}
Our work focuses on the extractive MRC setting, which aims to identify the correct answer span within a passage given a test question.

Interpretable methods for MRC have also seen much recent interest.  \citet{thayaparan2020explainability_survey} highlights the challenges facing MRC in terms of explainability and its impact on MRC performance. 
Several methods~\citep{https://doi.org/10.48550/arxiv.1412.1632, https://doi.org/10.48550/arxiv.1805.08092, Gravina2018CrossAF} have attempted to improve interpretability in MRC by identifying the supporting sentence for the answer. However, these methods rely on the availability of gold-supporting sentences, which may not always be present. \wenlong{We need gold-supporting sentences right?} Other methods utilize graph networks~\cite{https://doi.org/10.48550/arxiv.1911.02170,https://doi.org/10.48550/arxiv.1911.00484} and attention mechanisms to capture the attended parts of text or relations \cite{https://doi.org/10.48550/arxiv.1611.01603, Shao_2020}. In this work, we improve interpretability by providing a novel inference procedure that allows us to clearly attribute predictions to previously seen instances that were used in the decision-making process.


\paragraph{Case-based Reasoning.} 
Previous work \cite{cbr_akbc,das-etal-2020-probabilistic,cbr_subg,thai2022cbr, yang2023end} has demonstrated strong performance using case-based reasoning on knowledge graph reasoning tasks.
CBR has also been successfully applied to the task of semantic parsing \cite{das2021cbr, pasupat-etal-2021-controllable, awasthi2023structured}, where methods typically retrieve the logical forms of similar cases and pass them through a seq2seq model as input along with a target query.
Both settings, however, operate over structured spaces, 
where similarities between instances can more easily be determined by collecting and comparing symbolic patterns in the data, e.g., paths between nodes in a KG, or syntactic similarities in semantic parsing.
In this work, however, we adapt CBR to operate over unstructured text, and it is not obvious how existing methods can be re-used to work in this setting.

\paragraph{In-Context Learning.} In-context learning (ICL) is an emergent property of pre-trained language models \citep{brown2020language, min2022rethinking} that has shown remarkable recent success in several NLP tasks, particularly with large language models (LLMs) \citep{cheng2022binding, lewkowycz2022solving, dunn2022structured}. To make predictions, a model is simply prompted with a set of demonstrations for a target task along with a test instance to autoregressively generate the prediction. Recent work \citep{rubin2021learning, liu2021makes, li2023few, khattab2022demonstrate} has also shown strong performance by retrieving relevant demonstrations. This setting can be understood as a specific instantiation of the case-based reasoning framework, where the reuse step uses ICL instead of a fine-tuned model. ICL, however, has been shown to be oversensitive to the prompt \citep{chen2022relation}, besides leading to black-boxed inference, reducing the reliability of predictions. Problem decomposition and iterative prompting methods such as chain-of-thought \citep{wei2022chain} and least-to-most \citep{zhou2022least, drozdov2022compositional} attempt to address this issue by converting complex problems into intermediate steps. In contrast to methods reliant on emergent pre-training behavior, our work explicitly encodes the relational similarity hypothesis in a trained model to reuse exemplars for making predictions.


\paragraph{Retrieval-augmentation.} 
Retrieval forms a crucial component of most question-answering systems. For instance, retrieve-and-read is the \textit{de facto} paradigm for open-domain QA \cite{chen2017drqa,lewis2020rag,guu2020realm} -- models first retrieve evidence (passages) from a non-parametric memory for a given test question, followed by using a reader model to either extract or generate an answer conditioned on the retrievals. In contrast, our work retrieves similar \textit{questions} (as cases) instead of passages, in order to explicitly re-use their reasoning patterns. Beyond open-domain QA, prior work \citep{jiao-etal-2021-rept} has explored using retrieval during pre-training in order to enhance the distributional semantics learned by a language model for a specific task, such as MRC. In other work, \citet{kassner2020bertknn} proposed a retrieval-based method for improving cloze-style question answering by interpolating BERT predictions with a $k$-nearest neighbors search performed over representations of queries and words within relevant contexts.


% \subsection{Machine Reading Comprehension}

% \paragraph{Interpretable MRC}
% \june{Discuss the important of interpretability in MRC and how it was previously addressed.}

% \subsection{Case-Based Reasoning}

% \paragraph{Classic CBR}
% \june{Add one paragraph for classic CBR}

% \paragraph{CBR in NLP}
% \june{Add one paragraph for modern CBR. Citing work on CBR for KBQA, KBC and SP}

% \subsection{Learning by Demonstrations}

==> zz_fig_latent_rel.tex <==
\begin{figure}[t!]
    \centering
    \hspace*{-0.5cm}
    \includegraphics[width=7.5cm]{zzz_latentrel_f1.pdf}
    \caption{\textbf{F1 v/s Latent Relation Frequency}. We compare the test performance of \method\ v/s BLANC with respect to the frequency of latent relations of the test questions found in the training set.}
    \label{fig:latent-relation}
\end{figure}




==> zz_fig_traindev_loss.tex <==
\begin{figure}[H]
    \centering
\includegraphics[width=0.9\columnwidth]{zzz_traindev_loss_fig.pdf}
    %\hspace*{-10mm}
    \vspace*{-3mm}
    \caption{\textbf{Overview of machine-reading comprehension using CBR.} (upper) Given a test question, \method{} first retrieves similar cases from a memory of known (question, context, answer) triples. \method{} relies on the fact that contextualized answers to similar questions share semantic similarities with each other. (lower) \method{} then predicts as answer the span in the test context that has the highest similarity with the contextualized answer embeddings from the retrieved cases. 
    }
    \label{fig:traindev_loss}
    \vspace*{-8mm}
\end{figure}
